Texture Networks: Feed-forward Synthesis of Textures and Stylized Images

Gatys et al. recently demonstrated that deep networks can generate beautiful textures and stylized images from a single texture example. However, their methods requires a slow and memory-consuming optimization process. We propose here an alternative approach that moves the computational burden to a learning stage. Given a single example of a texture, our approach trains compact feed-forward convolutional networks to generate multiple samples of the same texture of arbitrary size and to transfer artistic style from a given image to any other image. The resulting networks are remarkably light-weight and can generate textures of quality comparable to Gatys~et~al., but hundreds of times faster. More generally, our approach highlights the power and flexibility of generative feed-forward models trained with complex and expressive loss functions.

==> scratch.tex <==
by matc that proposed an approach to stylized image and texture synthesis using deep networks have attracted a wide interest. They have demonstrated that artistic style and texture content can be captured remarkably well through measuring the correlations coefficients between convolutional maps at certain levels of a sufficiently deep pre-trained convolutional neural network (below we refer to this statistics as \textit{Deep Gram matrix}). Based on this observation, they demonstrated how prototype-based stylization and texture synthesis can be achieved by an optimization process that gradually changes the pixel values of a certain initial image in order to match the deep Gram matrix of the prototype.

While powerful, robust, and achieving remarkable results, the optimization-based approach of Gatys et al.~takes several minutes to generate a stylized image or texture of a small size. The image size is also limited by GPU memory, while generation using CPU is almost infeasible for large images. Achieving similar stylization and synthesis capability by a \textit{feed-forward process} would thus be highly desirable from practical point of view. Besides that, whether a feed-forward network can learn to impose style and generate complex textures, is an interesting question on its own right, which has not been addressed. 

Our work gives a positive answer to this question. We show that given a prototype image, a moderately-sized fully convolutional architecture can be trained to modify an arbitrary input image to match the deep Gram matrix of this prototype, and thus to impose the prototype style. Furthermore, for image stylization, the network can be simultaneously trained to preserve the \textit{content} of the input image (following \cite{todo} the content is captured by the representation of an image at a certain level of a deep pretrained CNN). 

After training, our \textit{stylizing networks} produce results that for most textures and artistic styles are visually similar to the results of \cite{TODO}. At the same time, after being trainined, stylizing networks take about two orders of magnitude less time and considerably (an order of magnitude) less memory compared to the Gatys~et~al.~approach. Being fully convolutional, stylizing networks can be applied to large images and synthesize large textures. Our approach also represents an interesting showcase of training conceptually-simple feed-forward architectures while using complex and expressive loss functions. We believe that other interesting results can be obtained using same principle.

{\bf Other related works.} Apart from \cite{Gatys1,Gatys2}, our approach can be related to several other works where feed-forward networks are trained with complex losses. Thus, adversarial networks \cite{Goodfellow14} and its variants \cite{Denton15,dcgan} train simple generator networks, while using parallelly-evolving discriminator networks to measure the loss. Below, we compare our approach and DCGan version of adversarial networks \cite{dcgan} for the task of texture generation. Another related approach are moment-matching generating networks of \cite{DziugaiteRG15}, and we further discuss this connection below.

% proposed a parametric method for texture synthesis based on convolutional neural networks (CNN). The texture is fed to VGG object recognition network \cite{DBLP:journals/corr/SimonyanZ14a} and feature maps at each layer are considered. It was shown that a texture image can be represented as a set of correlations between its feature maps. Thus having this representation one can iteratively optimize an image from noise to produce same representation as a given texture and converge to visually good texture. Unfortunately, there is no other metric for texture quality rather than human inspection but in authors opinion Gatys achieves state-of-the-art results on huge number of texture examples. 

% The extended version of texture synthesis algorithm for image stylizing utilizes similar principals.




% In this paper we propose using a parametric generator which learns to map samples from a simple distribution into textures directly minimizing the loss function proposed in Gatys. Therefore we are training neural network using only one example image. We learn generator to produce \texttt{256x256} images. However when trained the generator is able to produce a texture image of any size within a forward pass. We also extend texture generator to image stylizing network. This enables to stylize large images and HD video.


% GAN \cite{DBLP:conf/nips/GoodfellowPMXWOCB14}

% LAPGAN \cite{DBLP:journals/corr/DentonCSF15}

% Training generative neural networks via Maximum Mean Discrepancy optimization \cite{DBLP:journals/corr/DziugaiteRG15}

% Generative Moment Matching Networks \cite{DBLP:conf/icml/LiSZ15}

% Dosovitsky, chairs \cite{DBLP:conf/cvpr/DosovitskiySB15}

% DCGAN \cite{DBLP:journals/corr/RadfordMC15}

% Gatys, texture generation \cite{DBLP:journals/corr/GatysEB15}

% Gatys, artistic style \cite{DBLP:journals/corr/GatysEB15a}

% VGG  \cite{DBLP:journals/corr/SimonyanZ14a}

% batch normalization \cite{DBLP:conf/icml/IoffeS15}

% Adam \cite{DBLP:journals/corr/KingmaB14}

% image analogies \cite{DBLP:conf/siggraph/HertzmannJOCS01}

% MMD test is introduced in \cite{DBLP:conf/nips/GrettonBRSS06}

% We make the following contributions: 
% \begin{itemize}
% \item Explore structured loss [Gatys] for feedforward texture generation. We train a neural network using only one reference texture to generate similar textures. Because of convolutional nature the model is able to generate high resolution images with a single forward pass.
% \item We extend texture generator with content loss [Gatys, Artistic] making it possible to learn stylizing network.
% \item ? 
% \end{itemize}

% We consider statistics $\Phi(\x)$ built from a pre-trained \emph{convolutional} neural network $F(\x) = f_L \circ f_{L-1} \circ \dots \circ f_1(\x)$. As \emph{content} statistics in style transfer, we simply choose the output of the $l$-th layer of the neural network $F_l(\x) =  (f_l \circ \dots f_1)(\x)$:
% \begin{equation}\label{e:phicont}
%  \phicont(\x) = F_l(\x).
% \end{equation}
% As texture/style statistics we pool instead orderless information from local image features. For a convolutional network, $F_l(\x) \in \mathbb{R}^{H\times W \times C}$ is a tensor containing $H\times W$ spatial locations and $C$ feature channels. Denote by $F_l(\x|u,v) \in \mathbb{R}^C$ the column extracted at location $(u,v) \in \z_l$ (local feature). Then
% \begin{equation}\label{e:phitexone}
%  \phitex(\x;l) = \frac{1}{|\z_l|} \sum_{(u,v)\in \z_l}
%  \psi \circ F_l(\x|u,v).
% \end{equation}
% where $\psi : \mathcal{R}^C \rightarrow \mathcal{R}^d$ is a non-linear mapping increasing the expressiveness of the pooled statistics. For instance,~\cite{DBLP:journals/corr/GatysEB15,DBLP:journals/corr/GatysEB15a} pick the function
% \begin{equation}
%   \psi(\bv) = \bv \bv^\top
% \end{equation}
% computing the outer product of vector $\bv$. When averaged over spatial coordinates, this function computes the \emph{empirical correlation matrix} or \emph{Gram matrix} between local image features (below we refer to this statistics as \textit{Deep Gram matrix}). Their final texture descriptor is a stacking of such Deep Gram Matrices statistics
% \begin{equation}\label{e:phitex}
%  \phitex(\x) = \begin{bmatrix}
%  \sqrt{w_1}\operatorname{vec} \phitex(\x;1) \\ \vdots \\ \sqrt{w_L}\operatorname{vec} \phitex(\x;L)
%  \end{bmatrix}
% \end{equation}
% modulated by suitalbe non-negative weights $w_1,\dots,w_L$.


the content of the input image \y0






Let $L$ be a subset of the descriptor CNN layers and $F^l$ be the set of all feature maps at the layer $l \in L$. The corresponding Gram matrix $G^l$ is defined as a matrix of correlations between each pair of maps in $F^l$:
\begin{equation}
    G^l_{ij} = \sum_k F^l_{ik}F^l_{jk}
\end{equation}
Gatys shows that a set of Gram matrices $\{G^l\}, {l \in L}$ provides a description of the texture.  

To generate another texture sample $\bm{\hat x}$ we wish to minimize the squared L2 distance between the descriptions $G^l$ and $\hat G^l$:
\begin{equation}
    E^l = \sum_{l \in L} ||G^l - \hat G^l ||_2^2
\end{equation}

Finally, the loss is defined as a weighted sum of distances
\begin{equation}
    \mathcal{L}_{texture} = \sum_{l \in L}wE^l
\end{equation}
% where $w$ are corresponing weights.


The paper \cite{DBLP:journals/corr/GatysEB15a} described the following modification to turn texture generation method into stylization. Suppose an image $\bm{c}$ should be stylized with a style $\bm{x}$. Then select a set of layers $L_c$ and define
\begin{equation}
    \mathcal{L}_{content} = \sum_{l \in L_c} || F_c^l - \hat F_c^l ||_2^2
\end{equation}

The texture loss is now treated as a style loss and the stylization loss is then defined as 
\begin{equation}
    \mathcal{L}_{stylization} =\alpha \mathcal{L}_{style} + \beta \mathcal{L}_{content}
\end{equation}
where $\alpha$ and $\beta$ are the weighting factors. 

We use VGG object recognition CNN as a texture representation provider since it worked best for Gatys et al.




\subsection{Relation to generative moment matching networks}

MMD test is introduced in \cite{DBLP:conf/nips/GrettonBRSS06} cite somewhere ?
\cite{DBLP:journals/corr/DziugaiteRG15} this proposed first use MMD + NN 
\cite{DBLP:conf/icml/LiSZ15}  Generative Moment Matching Networks

Here we show the connection with generative moment matching networks \cite{DBLP:conf/icml/LiSZ15}. Texture loss can be seen as a case of maximum mean discrepancy measure between the set of feature map pixels from prototype and generated image. The feature maps $F^l$ can be seen as matrix $F^l \in \mathbb{R}^{d x wh}$ where $d$ is depth and $w$, $h$ corresponds to spatial dimensions. We refer to pixels as set of $d$ dimensional objects $F^l_{:,i}$. Let $X = \{F^l_{:,i}\}^{wh}_{i=1}$ be style image pixels and $Y = \{\hat F^l_{:,i}\}^{wh}_{i=1}$ pixels from generated image. It is clear that texture loss corresponds to second moment matching and can be seen as maximum mean discrepancy objective: 
\begin{align}
   \mathcal{L}_{texture} = \\
  = \sum_{l \in L} ||G^l - \hat G^l ||_2^2 = \\
  = || \frac{1}{wh}\sum_{i=1}^{wh} x_i x_i^T  - \frac{1}{wh} \sum_{i=1}^{wh} y_i y_i^T ||^2_2  = \\
  = || \frac{1}{wh}\sum_{i=1}^{wh} \phi(x_i)  - \frac{1}{wh} \sum_{i=1}^{wh}  \phi(y_i) ||^2_2  =\\
  = \mathcal{L}_{MMD^2}
\end{align}


% -----------------------------------------------------
% ------------------------- Texture model -------------
% -----------------------------------------------------
\subsection{Texture model}
Following the lines of [GAN] we decompose the image generation into two stages. At first a random sample $\bm{z}$ is drawn from a simple distribution $p$ and then transform the sample to image using generator $G(\bm{z}; W)$ with parameters $W$. We aim to learn a generator to minimize expected texture loss $\mathcal{L}_{texture}$:
% We aim to learn a generator $G(\bm{z})$ with parameters $\bm{w}$ which maps a simple to draw samples distribution $p$ into images, which are good in terms of texture loss $\mathcal{L}_{texture}$ based on texture $\bm{x}$. 
\begin{equation}
    \min_{\bm{w}} \mathbb{E}_{\bm{z} \sim p}\mathcal{L}_{texture}(G(\bm{z}; \bm{w}); \bm{x})
\end{equation}

To achieve this we iteratively minimize empirical loss using $N$ random samples $z_i \sim p, i =1,\dots,N$ at a time:
\begin{equation}
    \min_{\bm{w}} \sum_{i=1}^{N} \mathcal{L}_{texture}(G(\bm{z}_i; \bm{w}); \bm{x})
\end{equation}
To perform an optimization step we first draw samples $\{z_i\}_i^N$ from the prior distribution and generate samples $y_i = G(\bm{z}_i;W)$. The loss is evaluated within a forward pass of the VGG network and loss gradient w.r.t $y_i$ is computed during a backward pass. Note that the VGG parameters remain fixed. Gradient is then propagated through the generator and gradients w.r.t to parameters $\bm{w}$ are stored.




The convolution block is composed of three consecutive nonlinear convolutions with filter sizes \texttt{3x3}, \texttt{3x3} and \texttt{1x1}. To make training more efficient we use batch normalization \cite{DBLP:conf/icml/IoffeS15} between filters and nonlinearities. The number of filters in each convolution layer is from 8 to 40. precisely??? 

We use circular padding instead of zero padding to stop neural network glimpsing the edges. In fact, when using zero padding to process a noise vector the borders still remain determined. When generating a texture 

We use batch normalization \cite{DBLP:conf/icml/IoffeS15} layer before all depth concatenations to address the problem of unbalanced gradients. We tried to use L1 gradient normalization instead but results were slightly worse (is it ok to write like this ?). Some kind of branch gradients normalization happens to be a necessary condition for good convergence.   

We use simple nearest neighbour upsampling technique to enlarge feature maps. We tried strided full-convolution [DCGAN],\cite{long_shelhamer_fcn} but the results were not satisfying. 
